360{\deg} Stereo Image Composition with Depth Adaption

360{\deg} images and videos have become an economic and popular way to provide VR experiences using real-world content. However, the manipulation of the stereo panoramic content remains less explored. In this paper, we focus on the 360{\deg} image composition problem, and develop a solution that can take an object from a stereo image pair and insert it at a given 3D position in a target stereo panorama, with well-preserved geometry information. Our method uses recovered 3D point clouds to guide the composited image generation. More specifically, we observe that using only a one-off operation to insert objects into equirectangular images will never produce satisfactory depth perception and generate ghost artifacts when users are watching the result from different view directions. Therefore, we propose a novel per-view projection method that segments the object in 3D spherical space with the stereo camera pair facing in that direction. A deep depth densification network is proposed to generate depth guidance for the stereo image generation of each view segment according to the desired position and pose of the inserted object. We finally combine the synthesized view segments and blend the objects into the target stereo 360{\deg} scene. A user study demonstrates that our method can provide good depth perception and removes ghost artifacts. The per-view solution is a potential paradigm for other content manipulation methods for 360{\deg} images and videos.

==> sections/algorithm_discarded.tex <==
\iffalse
\section{Algorithm} 
The inputs of the method are a pair of stereo images of the object to be inserted, with a masked region-of-interest (RoI), and a stereo panoramic image pair as the target scene. The output is the composited image pair with correct depth perception of the inserted object for arbitrary view directions. The critical challenge is to find a proper binocular camera model to project inserted objects to target panoramic images while preserving correct depth perception. Another challenge lies in the generation of a complete and smooth depth map especially when the desired inserted 3D position is different from the original source position.

\subsection{Sparse 3D Reconstruction}
We first estimate the depth map of the foreground object and the region around the desired position of the target scene. For inserting the object into the stereo panoramic target scene represented by equirectangular projection, the user is required to specify the position and the size of object. We project the region-of-interest of the target scene to a planar image with a default FoV of 60\degree. If the source object is in a stereo panorama as well, we use a FoV of no less than 60\degree\ to cover the horizontal angle extent of the object when projecting the object into a planar stereo crop. We apply Li et al's sequence-to-sequence correspondence perspective deep model, named the STereo TRansformer (STTR), to estimate the disparity map from the stereo pairs \cite{li2020revisiting}.  %\textcolor{blue}{In addition, we could directlyse the provided ground truth depth value of an object, or apply any models to estimate the disparity or depth map.}

Using the predicted horizontal disparities between the input rectilinear stereo image pair, we can generate a depth map of the foreground objects based on camera parameters. Assume the focal length is $f$ and the baseline between the left and right camera is $B$, the depth values for the pixels can be calculated from its estimated disparity $d$:  $z = (f \times B) / d$.

Given a pixel $(p_x, p_y)$ on the left-view image with a size of $(W, H)$, we assumed a standard camera model located at the origin looking down the $z$-axis. The 3D coordinates of this point in the world coordinate system are obtained by: 
\begin{equation}
    (x, y, z)=\left(\frac{(p_x-W/2)\times z}{f}, \frac{(p_y-H/2)\times z}{f}, z\right),
\end{equation}
In the recovered sparse point cloud from the stereo pixels, we select the center point of the cloud as the object's reference point to place in the target scene and about which to make any transformations, such as scaling and rotation. It  also helps the user to correctly position the object in the target scene. Fig.~\ref{fig:f4_1_a} shows an example of a recovered 3D point cloud.

\subsection{\zfl{View Segmentation and Projection}}
\label{sec:ViewSeg}
\zfl{Having determined the transformations needed to meet the user's desires, including the size, orientation and position of the object, we obtain the 3D point cloud for the object that is to be inserted in the target scene. To address the aforementioned challenge of inconsistent depth, we segment the point cloud into different parts according to the individual points' directions from the user's position. As shown in Fig.~\ref{fig:view_dependent}(a), we first transform  world coordinates to a spherical coordinate representation by:}
\begin{equation}
\theta=\arctan\left(\frac{x}{z}\right)\ \ 
\phi=\arctan\left(\frac{y}{\sqrt[2]{x^{2}+z^{2}}}\right), \ \ 
\rho=\sqrt[2]{x^{2}+y^{2}+z^{2}}
\end{equation}
\zfl{Then we segment the point cloud according to the points' $\theta$-values: we split the range of $\theta$ into $N$ intervals, i.e., each interval covers a range of $\frac{2\pi}{N}$, and segment the points of the object based on the horizontal angle intervals in which they fall. 
}

\noindent\textbf{\zfl{View-Dependent Projection}} 
\zfl{In this step, we treat each segment of the point cloud with a virtual camera pair which focuses on the individual segment's center, and generates a series of view-dependent projected point clouds in their specific camera space (Fig. \ref{fig:view_dependent}(b)). %The depth map was in the spherical coordinate system, and we now need to transform it back to world coordinates before further processing.
The position and orientation of the user's binocular views are defined as follows. The virtual viewing camera pairs are located on the $xz$-plane of the world coordinate system, with up-vector along the positive $y$-axis. The initial position of each camera, $C_L^0$ and $C_R^0$ lands at the opposite sides of the origin on the $x$-axis with a distance $B$ between the two cameras, which are $C_L^0 = [-B/2, 0, 0]$, and $C_R^0 = [B/2, 0, 0]$, respectively. This initial pair's viewing directions are parallel to the positive $z$-axis. Given $N$ intervals, the system calculates the viewing direction of each interval $\theta_{i}$.}
\begin{equation}
    \theta_i= (2i+1)\pi/N-\pi
\end{equation}

\zfl{Then, the rotation matrix $R_i$ for such interval is computed based on the viewing direction, which is a rotation about $y$-axis by an angle $\theta_{i}$.}
%\begin{equation}
%    R_{i}=\begin{bmatrix}
%        \cos\theta_{i}  &0  &\sin\theta_{i} \\
%        0               &1  & 0 \\
%    -\sin\theta_{i}     &0  &\cos\theta_{i}
%    \end{bmatrix}
%\end{equation}
\zfl{We can define the desired position of $C_L^i$ and $C_R^i$ with associated viewing direction as:}
\begin{equation}
    C_L^i = R_{i} C_L^0,\ \
    C_R^i = R_{i} C_R^0
\end{equation}

\zfl{The projected 3D point cloud of each segment for both views, $Q_L^i$ and $Q_R^i$ with the specific camera matrix are expressed as}

\begin{equation}
    Q_L^i = [R_{i}| C_L^i] p_w = P_L^i p_w,\ \
    Q_R^i = [R_{i}| C_R^i] p_w = P_R^i p_w
\end{equation}

\zfl{Using the known intrinsic matrix of both cameras for a specific segment, we then project the point clouds to 2D depth maps. Note that the projected depth maps normally contains holes and gaps when the relative pose of the object to the camera changes. We thus need to estimate a dense depth map in the following steps to guide the generation of stereo RGB images for that view direction. Here, instead of just generating a depth map for the corresponding segment, we also generate the sparse depths for the neighboring regions in a certain field-of-view to facilitate the following dense depth map generation for each view.}


\subsection{\zfl{Per-view Image Generation and Fusion}}
\zfl{This step takes projected 2D sparse depth maps for each view direction as the input and returns the final composited stereo panoramic images. To ensure the perceived depths are correct when users are looking at different parts of the composited object, we propose to generate the dense depth maps and corresponding stereo RGB images based on the projected point clouds for each view separately. The stereo images for each view are then fused together to generate the final left and right panoramas. 
}

\subsubsection{\zfl{Deep Depth Densification}}
\zfl{Given a desired pose of object, the projected depth maps could be very sparse for each view direction of the stereo camera pairs. We primarily attempted to directly fill the missing 2D pixels on the depth map by morphological interpolation, !!TO CITE!!. However, the interpolation-based method only works when the pose changes are subtle so that the missing points can easily find valid depth values in their neighborhoods. If the object has a relatively large scaling and rotation, the valid points would be too sparse to provide sufficient reference values for the missing pixels to interpolate. Moreover, since we need to generate dense depth maps for each view, the long running time of morphological interpolation will cause a large negative impact on the efficiency of our method. Thus, we propose to utilize deep neural networks to generate dense depth maps efficiently with a higher visual quality especially for objects with sharp geometry features. Particularly, to get rid of the effect of the distortion in the equirectangular representation on the learning process, our deep model works in the 2D rectilinear image domain.
}

\zfl{
\textbf{Architecture}
We build a convolutional generative network that takes a projected sparse depth map as input and predicts dense valid depths for the target object. 
As shown in FIGURE XXX, a 2D sparse depth map goes through a U-Net-like architecture to produce a densified depth map. More specifically, we employ the following two learning schemes to improve the quality of generated depth maps: First, we explicitly predict a mask that indicates whether a pixel belongs to the target object in the final image, helping the network to learn whether a pixel should have a valid depth value. Second, we let the decoder to learn from multi-scale masks to have a better capability of reconstructing the object' geometry structure. For each scale level, we use a separate convolutional layer to estimate the mask, which is then processed and fed to the layers of the next scale level to provide higher-scale contextual information. In our experiment, the above schemes are shown to be effective especially for improving the depth map quality for those regions with large sparsity.    }

\begin{figure*}[t]
 \includegraphics[width =\linewidth]{figures/network.pdf}
 \caption{\zfl{Network}}
 \label{fig:view_dependent}
\end{figure*}
\zfl{\textbf{Dataset} 
Since it is tedious and laborious to collect a real-world stereo dataset with multiple views of the objects for training the above network, we build a synthetic dataset with ground truth depth maps of rendered objects. We use Unity3D to render RGB images and their associated dense depth maps with different positions, scales, and orientations. We select XXX objects from XX classes of 3D shapes in the ShapeNet dataset, covering a variety of categories of furniture, vehicle, housewares, and animals. For each object, we render XXX different poses, producing XXX dense depth maps $\{D_k\}$ and their corresponding masks $\{M_k\}$. The original pose for each object is chosen as its reference pose and a sparse point cloud $P_0$ is reconstructed from its depth map $D_0$. The transformations $\{T_k\}$ between the other poses and the reference pose are then applied on $P_0$ to generate the sparse depth maps $\{\hat{D}_k\}$. We use the sparse depth map $\hat{D}_k$ to simulate the input data for the real-world use case, where the sparse depth map can be generated from transforming the reconstructed point clouds from the original stereo object to the desired 3D orientation and position. The corresponding dense map $D_k$ and mask $M_k$ can be used to supervise the learning process.     
}

\zfl{
\textbf{Training Procedure }
The neural networks are trained to fill the gaps and missing points while preserving the important geometry structures for a sparse depth map. We use the following losses in the training procedure:
}
\zfl{
1. The reconstruction loss $L_r$. It is a L2 loss applied on the predicted depth map, defined as:}
$$L_r = \sum^K_{k = 1}|D_k - F_d(\hat{D}_k)|_2$$
\zfl{where $F_d(\hat{D}_k)$ represents the predicted dense depth map from the sparse map $\hat{D}_k$.}
\zfl{
2. The mask loss $L_m$. It is the loss of the side output masks of different scales, to ensure a proper object shape for the novel pose, which is defined as:}
$$L_m = \sum^K_{k = 1} \sum^L_{l = 0} |M^l_k - F^l_m(\hat{D}_k)|$$
\zfl{where $M^l_k$ is the ground truth mask for the scale $l$ and $F^l_m(\hat{D}_k)$ is the predicted mask for scale $l$. Finally, we add a perceptual loss $L_p$ applied on the depth map to produce better details, making the overall loss as:}
$$L = \lambda _rL_r + \lambda _mL_m + \lambda _pL_p$$
\zfl{By default, we set $\lambda _r = 0.3, \lambda _m = 0.3$, and $\lambda _p = 0.4$ as the weights for different terms. We split our datasets into a training set of $XXXX$ images and a test set of $XXX$ images. We further use 20\% of the training set as the validation data. We train our network by 100 epochs or make an early-stop when the losses on the validation data stop declining.}

\zfl{We show some results of our method and other alternatives in Figure XXX. It is hard for interpolation-based methods to properly fill the missing pixels in the boundary parts, since the transformed points can be very sparse in the projected depth map and can not form any continuous line structures to wrap up the object. The utilisation of the mask losses not only avoids the depth value "leaking" to pixels that should be outside of the object's contours, but also makes the network more confident when estimating the depth values for pixels with strong geometry features. Using such a network, we are able to promptly produce all the dense depth maps where the camera pairs are focused on the centers of different 3D point segments. }

\subsubsection{\zfl{Final Stereo Panorama Generation}}
\zfl{
Given the dense depth map for each view direction, we re-project each pixel to the original input stereo image to obtain its color value. In the original image, the system applies alpha matting CITATION XXX to generate soft edges for composition. To ensure a seamless composition, we also create an associated alpha mask by copying the alpha value of each referred original pixel. 
For all the $N$ segments of the point cloud, we thus obtain $N$ stereo image pairs $\{I^r_n, I^l_n\} (n = 1, 2, ..., N)$ with their alpha masks. To accelerate the process, we only require that the depth map and stereo RGB images can cover the involved part of the object and its neighboring region, since the other parts out of the specified view range will not be used in the final result generation. Moreover, feeding the sparse depth map of the 
entire object does not produce a better quality in our experiments, but reduces the resolution of the focused segment of the object in the resultant image. 

We compose the synthesized left and right views of each segment to the left and right views of the target panorama respectively. For stereo panoramas captured by 360\degree\ cameras, we obtain their depths using the 360\degree\ depth estimation method proposed in CITATION XXX to align the 3D scenes of the target and the source images. Then with the camera model introduced in Sec.~\ref{sec}, for each pair of the cameras $(C^i_L, C^i_R)$, we use its view direction and the interval $\theta_i$ to obtain the affected pixels in the left and right views of the target panorama. Since the columns of an equirectangular image are naturally the pixels of different horizontal viewing angles, we just need to calculate the affect columns and project those spherical pixels to the 2D image plane of the synthesized image $I^r_i$ or $I^l_i$ to find the pixels to overwrite the original colors. The pixels' alpha values will be used to ensure that only valid pixels will be used and seamlessly blended. We find that a larger number of segments always means a better visual quality. Therefore, in our default settings, the viewing angle intervals are decided by the horizontal resolution of our target panoramic images and normally set as the viewing angle represented by a single column. For example, for a 4K resolution panorama (4096*2048), our interval is 360\degree\ / 4096 = 0.08\degree. }

\zfl{
We could also use larger intervals to save computational time. In that case, if the segment number is too small, there will be visible gaps between neighboring composited segments. We fuse them by applying a deformation method that is based on Moving Least Squares \cite{schaefer2006image}. Suppose there is a gap between adjacent segments $S_1$ and $S_2$, we define $2n$ control points along the left and right borders of a narrow band at the right end of $S_1$ and the left end of $S_2$. Then we fix the left column of control points of $S_1$ and the right column of the control points of $S_2$, and drag the right column of $S_1$'s control points and the left column of $S_2$'s to the middle of the gap and let the corresponding points to be coincident as they were in the unsegmented depth map. Most parts of the image retain the consistent disparities generated by the view-dependent rendering, with the intention that the joins between the different parts are imperceptible. 
Fig. \ref{fig:fusing_comparison} shows the difference between using this fusion technique and the obvious join that results from simply combining the segments together when the segment is too large. Finally, we could compare the depth of the inserted object with that of the panorama to determine the occlusion relationship for better composition. 
}

\begin{figure}[t]
 \includegraphics[width =\linewidth]{figures/View_dependent.pdf}
 \caption{Spherical coordinate representation and view-dependent projection. }
 \label{fig:view_dependent}
\end{figure}

\iffalse
\subsection{View Segmentation}
Having determined the transformations needed to meet the user's desires, including the size, orientation and position of the object, we obtain the 3D point cloud for the object which is to be inserted in the target scene. To address the aforementioned challenge of inconsistent depth, we segment the point cloud into different parts according to the individual points' directions from the user's position. As shown in Fig.~\ref{fig:view_dependent}(a), we first transform  world coordinates to a spherical coordinate representation by:
\begin{equation}
\theta=\arctan\left(\frac{x}{z}\right)\ \ 
\phi=\arctan\left(\frac{y}{\sqrt[2]{x^{2}+z^{2}}}\right), \ \ 
\rho=\sqrt[2]{x^{2}+y^{2}+z^{2}}
\end{equation}
Then we segment the point cloud according to the points' $\theta$-values: we split the range of $\theta$ into $N$ intervals, i.e., each interval covers a range of $\frac{2\pi}{N}$, and segment the points of the object based on the horizontal angle intervals in which they fall.

Note that the transformed spherical coordinates need to be projected in an equirectangular manner in order to generate the commonly used panoramic stereo image format, which can only produce sparse pixels. The sparsity of the projected points are greatly influenced by several factors, for example, the value of the latitude where the foreground lands, and the modified size and orientation of the object. If there are too many missing pixels along the boundary of each part, extra challenges emerge in the later interpolation and fusion step when synthesizing the complete dense images. Therefore, in this step, we make  extra refinements to the point cloud before segmentation. Since the point positions in the equirectangular projection from the 3D points to a sphere centered at the origin would be quite similar with the final results, we densify the  depth map and pixel mask generated in such a method to achieve a more complete point cloud. 

Given a sparse depth map (shown in a normalized-visualization form in Fig. \ref{fig:f4_1_b}), we investigated two ways to fill the sparseness: (i)~morphological operatios and (ii)~interpolation.  We investigated the use of simple open and close morphological operations defined in OpenCV (Fig. \ref{fig:f4_1_c}), but they generate discontinuous and unrealistic depth maps: the filled-in values generate blocky artifacts in the result. So we propose instead to interpolate missing depths using existing depth values in a local area. As shown in Fig.~\ref{fig:f4_2}, we define a cross kernel $T$ for each pixel. It computes the depth value of a missing pixel $(i,j)$ as follows:
\begin{equation}
    D_{(i,j)} = \frac{1}{k}\sigma M(m,n) T(m,n) D_{m,n}
\label{Equ:interpolation}
\end{equation}

Where D is the depth map, $M$ is the binary mask recording which pixels are missing, and $k$ is the valid pixel number covered by $T$. Our template-based interpolation method generates a better quality result (Fig. \ref{fig:f4_1_d}). In the example, we can see the gradual colour change at both sides which shows the depth is slightly increased from the middle to the two sides, generating a more realistic depth distribution. For points generating larger missing areas, one round of interpolation may not be able to cover all the pixels. In all our examples, it normally takes 2--3 iterations to fill the depth values. 


\begin{figure}
\centering
    \begin{minipage}{.23\textwidth}
      \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/algorithm/movie280.png}
        \caption{Recovered 3D point cloud}
        \label{fig:f4_1_a}
      \end{subfigure}%
  \end{minipage}
  \hfill
     \begin{minipage}{.23\textwidth}
      \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/algorithm/sparse_depthmap.png}
        \caption{Sparse after spherical projection}
        \label{fig:f4_1_b}
      \end{subfigure}\\
      \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/algorithm/morpho_dense_depthmap.png}
        \caption{Morphological completion}
        \label{fig:f4_1_c}
      \end{subfigure}\\
      \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/algorithm/inter_dense_depthmap.png}
        \caption{Interpolation-based completion}
        \label{fig:f4_1_d}
      \end{subfigure}%
    \end{minipage}
  \caption{\zfl{To replace by depth maps and alpha masks generated by our network.} Depth map completion in the spherical domain}
  \label{fig:f4_1}
\end{figure}

\begin{figure}
\centering
  \begin{subfigure}[t]{.18\textwidth}
    \centering
    \includegraphics[width=3cm, height=3cm]{figures/algorithm/m0.png}
    \caption{Cross Kernel}
    \label{fig:f4_2_a}
  \end{subfigure}
  \begin{subfigure}[t]{.18\textwidth}
    \centering
    \includegraphics[width=3cm, height=3cm]{figures/algorithm/m1.png}
    \caption{Sparse depth map}
    \label{fig:f4_2_b}
  \end{subfigure}
  \begin{subfigure}[t]{.18\textwidth}
    \centering
    \includegraphics[width=3cm, height=3cm]{figures/algorithm/m2.png}
    \caption{Iterating}
    \label{fig:f4_2_c}
  \end{subfigure}
  \begin{subfigure}[t]{.18\textwidth}
    \centering
    \includegraphics[width=3cm, height=3cm]{figures/algorithm/m3.png}
    \caption{Dense depth map}
    \label{fig:f4_2_d}
  \end{subfigure}
  \vspace{-4mm}
  \caption{\zfl{To replace by deep learning-based pipeline} A template is applied here as an example of showing how the our depth interpolation works. The yellow squares show the weights of each tile in the kernel. The sparse depths are shown in gray, and empty pixels are shown as blue. We take the mean of the valid values covered by the kernel to fill the sparse depth map iteratively.}
  \label{fig:f4_2}
\end{figure}




\subsection{View-Dependent Projection}
This step takes the results from the previous step where we have a segmented dense depth map with region-of-interest as the input, and we treat each segment with a virtual camera pair which focuses on the individual segment's center. The outputs are a series of view-dependent projected point clouds in their specific camera space (Fig. \ref{fig:view_dependent}(b)). The depth map was in the spherical coordinate system, and we now need to transform it back to world coordinates before further processing.

The position and orientation of the user's binocular views are defined as follows. The virtual viewing camera pairs are located on the $xz$-plane of the world coordinate system, with up-vector along the positive $y$-axis. The initial position of each camera, $C_L^0$ and $C_R^0$ lands at the opposite sides of the origin on the $x$-axis with a distance $B$ between the two cameras, which are $C_L^0 = [-B/2, 0, 0]$, and $C_R^0 = [B/2, 0, 0]$, respectively. This initial pair's viewing directions are parallel to the positive $z$-axis. Given $N$ intervals, the system calculates the viewing direction of each interval $\theta_{i}$.
\begin{equation}
    \theta_i= (2i+1)\pi/N-\pi
\end{equation}

Then, the rotation matrix $R_i$ for such interval is computed based on the viewing direction, which is a rotation about $y$-axis by an angle $\theta_{i}$.
%\begin{equation}
%    R_{i}=\begin{bmatrix}
%        \cos\theta_{i}  &0  &\sin\theta_{i} \\
%        0               &1  & 0 \\
%    -\sin\theta_{i}     &0  &\cos\theta_{i}
%    \end{bmatrix}
%\end{equation}
We can define the desired position of $C_L^i$ and $C_R^i$ with associated viewing direction as:
\begin{equation}
    C_L^i = R_{i} C_L^0,\ \
    C_R^i = R_{i} C_R^0
\end{equation}

The projected 3D points cloud of each segment for both views, $Q_L^i$ and $Q_R^i$ with the specific camera matrix are expressed as
\begin{equation}
    Q_L^i = [R_{i}| C_L^i] p_w = P_L^i p_w,\ \
    Q_R^i = [R_{i}| C_R^i] p_w = P_R^i p_w
\end{equation}






\subsection{Refinement and Fusion}
\begin{figure}
\centering
  \begin{subfigure}[t]{.23\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/algorithm/90_left_nostretch.png}
    \caption{Left view without fusing}
    \label{fig:f4_3_a}
  \end{subfigure}
  \begin{subfigure}[t]{.23\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/algorithm/90_right_nostretch.png}
    \caption{Right view without fusing}
    \label{fig:f4_3_b}
  \end{subfigure}
  \begin{subfigure}[t]{.23\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/algorithm/90_left_stretch.png}
    \caption{Left view with fusing}
    \label{fig:f4_3_c}
  \end{subfigure}
  \begin{subfigure}[t]{.23\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/algorithm/90_right_stretch.png}
    \caption{Right view with fusing}
    \label{fig:f4_3_d}
  \end{subfigure}
  \vspace{-4mm}
  \caption{View fusion example. To better demonstrate the gaps between different parts, we insert a synthetic object with obvious markers.}
  \label{fig:fusing_comparison}
\end{figure}

\zfl{To rewrite } This step takes the projected points as the input and returns the final composited results by applying several techniques to refine the details of the input. The system applies alpha matting to generate soft edges for composition, and also implements homographical warping to achieve proper RGB values in the distorted foreground according to users' needs. Since the target scene is in the equirectangular form, sometimes there will be multiple pixels in the target scene matching to the same pixel in the source image. Therefore, we use bi-linear interpolation to avoid repeating pixels when retrieving based on 3D positions (this intermediate result is shown in Fig. \ref{fig:view_dependent} (c)). The segments after the projection may generate new artifact, since the density is not guaranteed by the view-dependent projection from 3D space. We further refine the image by using a depth-aware interpolation method to fix those missing pixels in each view. Here, we interpolate the depth values
%using Equ. \ref{Equ:interpol} again,
and use the point's depth to retrieve its color in the source image with the help of bi-linear interpolation.

\begin{figure*}
  \includegraphics[width =0.96\linewidth]{figures/results/big_results.pdf}
    \vspace{-3mm}
    \caption{Results of the proposed method (all in stereo form). Left to right: foregrounds and their target scene, equirectangular composition results, and the occlusion mesh view of the results in VR.}
    \vspace{-4mm}
  \label{fig:f4_1}
\end{figure*}

The next step takes the refined results of each segment and fuses them by applying a deformation method that is based on Moving Least Squares \cite{schaefer2006image}. Suppose there is a gap between adjacent segments $S_1$ and $S_2$, we define $2n$ control points along the left and right borders of a narrow band at the right end of $S_1$ and the left end of $S_2$. Then we fix the left column of control points of $S_1$ and the right column of the control points of $S_2$, and drag the right column of $S_1$'s control points and the left column of $S_2$'s to the middle of the gap and let the corresponding points to be coincident as they were in the unsegmented depth map. Most parts of the image retain the consistent disparities generated by the view-dependent rendering, with the intention that the joins between the different parts are imperceptible. 
Fig. \ref{fig:fusing_comparison} shows the difference between using this fusion technique and the obvious join that results from simply combining the segments together. Finally, we compare the depth of the inserted object with that of the panorama to determine the occlusion relationship for better composition. 





\subsection{Coordinates Transformation}
In this step, we first transform the foreground objects' coordinates with their estimated depths value from the pixel space (2D image plane) to the world space (3D points cloud). Then we adjust the size, orientation, and position of the foreground objects in world space by applying the transformation matrices. Finally, we assuming the equirectangular image (target image) is wrapped onto a sphere, and projecting the transformed 3D foreground objects onto that sphere. In another word, transform the foreground objects' coordinates from the Cartesian coordinate system to the sphere coordinate system.

As we have complement the depth dimension of our 2D stereo source input images in the previous step, we can first convert those pixel coordinates in the projection space to the camera space because any 3D point can be expressed by multiple coordinate systems. Fig. \ref{fig:f3_2_a} shows how the coordinates transform from the projection space to the camera space or vice versa. The camera coordinate system is defined as the $X_{c}, Y_{c}, Z_{c}$ axis in the figure. Whereas the pixel coordinate system shows a pair of integers (x and y) giving the column number and the row number of a digital image. In addition, we need to move the original point of the pixel coordinate system aligned with the z-axis, and also invert the y-coordinate of the point. As the depth ($z_{c}$) for each point in multiple coordinate systems is consistent, and assume the optical center of the camera locates at the origin of the Cartesian coordinate system, a given point ($x_{w}$, $y_{w}$, $z_{w}$) in the world space can be computed as follows,
\begin{equation}
    (x_{w}, y_{w}, z_{w})=(\frac{(x-\frac{w}{2})\times z_{c}}{f}, \frac{(y-\frac{h}{2})\times z_{c}}{f}, z_{c}),
\end{equation}
where x and y are the number of the specific column and row of the source image, and h and w mean the resolution of height and width of the source rectilinear image. The points cloud of the foreground objects in Cartesian coordinate system are shown in Fig. \ref{fig:f3_3_b}.

After we get the points cloud of the foreground object in the world space, we can apply the transformation matrices to achieve the object transformation for adjusting the position, rotation, or scale when it is compositing to the target scene with the consistent geometry relationship inside this object. We select the most bottom then rightmost point of the object as the original point for changing the coordinates to the object space because this point is usually where the object lands in the target scene. Then, we are going to multiply those object space coordinates by the transformation matrices to get transformed 3D points cloud in the world space, which is computed as follows, 
\begin{equation}
    V_{world}=M\times V_{model},
\end{equation}
where M is equal to the result of the translation matrix, rotation matrix, and scale matrix multiplied together in this order, in addition, all the calculations are under homogeneous coordinates.

\begin{figure}[h]
\begin{subfigure}{0.49\linewidth}
\includegraphics[width=\linewidth, height=4.2cm]{figures/pixel2world.png} 
\caption{Transforming coordinates from the pixel space to the camera (world) space}
\label{fig:f3_2_a}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
\includegraphics[width=\linewidth, height=3.8cm]{figures/spherical_coord.png}
\caption{A given point in the world and spherical coordinate system \red{Change to a picture where the sphere is kept, and put aside a real equirectangular panoramic image to show what the spherical coordinates mean.}}
\label{fig:f3_2_b}
\end{subfigure}
\caption{Coordinate system transformation}
\label{fig:f3_2}
\end{figure}

As the target scene is an equirectangular image, which warps on the sphere. We now need to project the pre-processed 3D points cloud onto a sphere. The reason we cannot directly clone the foreground object to the equirectangular image is that the objects obtained by the equirectangular image appear to be distorted. The equirectangular image directly maps the latitude and longitude of a sphere on the horizontal and vertical Cartesian coordinate system, which covers 360 degrees horizontally and 180 degrees vertically. Objects at the centre of the image will be compressed and stretched at the zenith and nadir along the latitude. So, we need to project those 3D points cloud onto the sphere to get a projection texture of the foreground objects with a correct distortion.


We now define the spherical projection using the following terms. In Fig. \ref{fig:f3_2_b}, we use rho ($\rho$), phi ($\phi$) and theta ($\theta$) to indicate the position of the point P under the spherical coordinate system, where rho is the distance between the P and the original point, rho and phi are the angles between the y-axis and z-axis to the direction of the point P, respectively. Rho, theta, phi and their respective position on the equirectangular image can be computed as follows,
\begin{equation}
    \rho=\sqrt[2]{x^{2}+y^{2}+z^{2}},
\end{equation}
\vspace{-6mm}
\begin{equation}
    \phi=\arctan\left(\frac{y}{\sqrt[2]{x^{2}+z^{2}}}\right),
\end{equation}
\vspace{-3mm}
\begin{equation}
\theta=\arctan\left(\frac{x}{z}\right),
\end{equation}
\vspace{-3mm}
\begin{equation}
(i, j)=(\frac{\left(\phi+\frac{\pi}{2}\right)\times H}{\pi}, \frac{\left(\theta+\pi\right)\times W}{2\pi}),
\end{equation}
where i and j are the row, and column number in the equirectangular image, and H and W are the resolution of height and width of the equirectangular image. The angle range of phi is from $\frac{\pi}{2}$ to $-\frac{\pi}{2}$, and theta is from $\pi$ to $-\pi$. Fig. \ref{fig:f3_3_c} gives examples of the 3D points projected onto the sphere.

\subsection{Depth and Mask Refine}
This step aims at refining the depth map and the alpha mask of the sphere projected foreground objects. From the Fig. \ref{fig:f3_3_c}, we can see that the projected 3D points cloud become sparse or have some outliers at some specific region. We implement the morphological techniques to tackle this problem. For example, we first use the ‘Opening’ operation to remove noise, which is another name of erosion followed by dilation. Then, apply ‘Closing’, which is the reverse version of ‘Opening’ (dilation followed by erosion) to fill small holes inside the foreground objects. The results of the dense depth map and alpha mask are shown in Fig. \ref{fig:f3_3_d}.
\fi

\iffalse
In this step, the left and right spherical projections of the foreground objects are blended into the corresponding background equirectangular images with an appropriate disparity and perspective scaling. We use alpha matting and gradient-domain algorithm to make the colour appearance of the composited foreground objects integrate well into the target scene. The composition results appear in a high quality and achieve the stereo visual pleasing.

For computing a exact disparity, we need to first determine the baseline of the stereo camera of capturing the target scene equirectangular images. The baseline is the physical distance between the parallel cameras, and it can be defined in the following terms (see Fig. \ref{fig:f3_5}). $C_{l}$ and $C_{r}$ are the panoramic cameras that are horizontally aligned on the x-axis, and $x_{l}$ and $x_{r}$ indicate their position under the world coordinate, respectively. Point P is the matching point that we get by applying the oriented FAST rotated BRIEF (ORB) detector, and $x_{p}$ is its position on the x-axis. $\theta_{l}$ and $\theta_{r}$ are the angles between the z-axis and the vector from the camera to the point P. Depth Z can be considered as physical distance of Point P orthogonality of the x-axis, and the baseline can be computed as follows,                              
\begin{equation}
    B=\mid\tan(\theta_{l})-\tan(\theta_{r})\mid\times\:z, \:if \:x_{p}<x_{l}\: or\:x_{p}>x_{r},
\end{equation}
\vspace{-6mm}
\begin{equation}
    B=\mid\tan(\theta_{l})+\tan(\theta_{r})\mid\times\:z, \:if \: x_{l}\leq x_{p} \leq x_{r}.
\end{equation}

After we acquire the baseline of the stereo cameras, we can calculate the disparity angle of each point according to the position of the left camera to compute an appropriate right-eye view. We overcome a challenge which is proposed by Tong et al. \cite{tong2012stereopasting}, they describe the challenge as their stereoscopic composition algorithm is not working well when dealing with a large area of occlusion or perspective difference between foreground objects and the backgrounds because the disparities of the 3D background are recovered incorrectly. For our image composition method, we consider more factors such as the geometric structure of the foreground objects and depth information of the target scene. In addition, we also achieve a authentic occlusion view caused by viewing angles and a dynamic disparity at different position along the y-axis in the equirectangular images. The disparity angle according to the left camera is shown as follows,
\begin{equation}
    \theta_{r}=\arctan(\tan(\theta_{r})\times z\;-B,\;z).
\end{equation}

Finally, we apply alpha matting and gradient-domain method to composite the texture of the spherical projected foreground objects to the target scene, and the composition results are natural and showing good generalisation and compatibility across different scenes.

\begin{figure}[hbt!]
 \centering
 \includegraphics[width = 0.75\linewidth]{figures/disparity.png}
 \caption{Spherical angle disparity with a horizontal (latitude) cross-section.}
 \label{fig:f3_5}
\end{figure}
\fi

\iffalse
\begin{figure}[h]
\begin{subfigure}{0.49\linewidth}
\includegraphics[width=\linewidth]{figures/bilinear_comparison/bags_left_final_b.png} 
\caption{Bilinear interpolation mapping}
\label{fig:f3_4_a}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
\includegraphics[width=\linewidth]{figures/bilinear_comparison/bags_left_final_nob.png}
\caption{Approximate mapping}
\label{fig:f3_4_b}
\end{subfigure}

\caption{Computing RGB with different mapping method}
\label{fig:f3_4}
\end{figure}
\fi
